Interference Among First-Price Pacing Equilibria: A Bias and Variance Analysis

Online A/B testing is widely used in the internet industry to inform decisions on new feature roll-outs. For online marketplaces (such as advertising markets), standard approaches to A/B testing may lead to biased results when buyers operate under a budget constraint, as budget consumption in one arm of the experiment impacts performance of the other arm. To counteract this interference, one can use a budget-split design where the budget constraint operates on a per-arm basis and each arm receives an equal fraction of the budget, leading to ``budget-controlled A/B testing.'' Despite clear advantages of budget-controlled A/B testing, performance degrades when budget are split too small, limiting the overall throughput of such systems. In this paper, we propose a parallel budget-controlled A/B testing design where we use market segmentation to identify submarkets in the larger market, and we run parallel experiments on each submarket. Our contributions are as follows: First, we introduce and demonstrate the effectiveness of the parallel budget-controlled A/B test design with submarkets in a large online marketplace environment. Second, we formally define market interference in first-price auction markets using the first price pacing equilibrium (FPPE) framework. Third, we propose a debiased surrogate that eliminates the first-order bias of FPPE, drawing upon the principles of sensitivity analysis in mathematical programs. Fourth, we derive a plug-in estimator for the surrogate and establish its asymptotic normality. Fifth, we provide an estimation procedure for submarket parallel budget-controlled A/B tests. Finally, we present numerical examples on semi-synthetic data, confirming that the debiasing technique achieves the desired coverage properties.

==> commands.tex <==

\newcommand{\rev}[0]{\textrm{Rev}}
\newcommand{\nsw}[0]{\textrm{NSW}}
\newcommand{\tod}{{ \,\overset{{\,d\,\,}}{\rightarrow}\, }}

==> experiment_v0.tex <==
\section{Experiment} \label{sec:exp}
To evaluate our proposed framework and debiased estimator, we run both fully synthetic and semi-synthetic simulations to check if the proposed estimator for beta and revenue are indeed less biased as well as the coverage of the proposed estimator.

\subsection{Fully synthetic experiments} \label{ssec: simulation}
In the fully synthetic experiments, we simulate 10 buyers and 1000 \emph{good} items in two submarkets, with a varying number of \emph{bad} items (up to 500) in order to study the effect of the contamination parameter $\alpha$. For each $\alpha$, we randomly sample a budget from a uniform distribution for each buyer, and compute ${\boldsymbol \beta}^*$ and $\REV^*$ from the limit pure market $\cM_0$ with a uniformly distributed value function in each submarket. To check if the debiased surrogate reduces bias, we compute ${\boldsymbol \beta}^*\sa$ and $\REV^*\sa$ from the limit market with interference $\cM\sa$ and their surrogates, $\widetilde{\boldsymbol \beta}^*$ and $\widetilde\REV^*$. We look at the normalized bias for the surrogate, defined as $\| \betastt - \betast \|_2 / \| \betast \|_2$ for pacing multipliers and as $|\widetilde\REV^* / \REV^* - 1|$ for revenue, and similarly defined for the limit quantities. \cref{fig:sim_bias} shows the normalized bias curves as a function of $\alpha$.
It can be seen that the magnitude of the bias increases with $\alpha$, for both the variables in the limit market with interference $\cM\sa$ and their debiased surrogates. We see that the bias of the debiased surrogates is indeed much smaller than the contaminated limit quantities.
\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{parallel_ab_normalized_bias_full_synthetic.eps}
	\caption{Normalized bias (in percent of true value) as a function of $\alpha$ in fully synthetic experiments. $\widetilde{\boldsymbol \beta}^*$ and $\widetilde\REV^*$ are the debiased surrogates for pacing multiplier and revenue in the limit market with interference $\cM\sa$. }
	\label{fig:sim_bias}
\end{figure}

Next, we check the coverage of the proposed variance estimator. For each $\alpha$ and each budget sample, we run 100 simulations in the following way: We sample items (or their values for each buyer) considering two submarkets and bad items. We then run the finite FPPE with bad items and obtain a baseline estimate for pacing multiplier and revenue without applying the debiasing procedure. Then, we apply the debiasing procedure to compute the debiased estimates. For each simulation, we check if the debiased surrogate is within the confidence interval of the debiased estimator. Finally, we aggregate them to compute the estimated coverage of the estimator. The results for both pacing multiplier and revenue are shown in \cref{tab:full_synthetic_revenue_coverage}. For the coverage of $\widehat{\boldsymbol \beta}$, we first compute the coverage of each component and report only the average in the table. It is shown that $\widehat{\boldsymbol \beta}$ is slightly over-covered. We found that the over-coverage is mainly due to the over-estimation of the estimator's variance. For revenue, we construct the CI using the two approaches as mentioned in~\cref{sec:res_rev}: one based on \cref{eq: revenue_ci} and the other using parametric bootstrap based on the estimated asymptotic distribution of $\widehat{\boldsymbol \beta}$ (with "(b)" in the column names). First of all, we show in \cref{fig:sim_convergence} that both CIs converges to the true value from the limit market with interfrence $\cM\sa$ as the number of items goes to infinity. Then, in ~\cref{tab:full_synthetic_revenue_coverage}, we show that the bootstrap CI width is much smaller compared to that from \cref{eq: revenue_ci}. However, both CIs are over-covered, higher than the nominal level (95\%). It is expected though that the CI from \cref{eq: revenue_ci} is relatively large and hence conservative since it uses the min and max of each $\beta_i$, hence likely living outside of the confidence region ($n$-dimension ellipsoid) for $\widehat{\boldsymbol \beta}$ and leading to over-coverage. For the bootstrap CI, it requires enough bootstrap samples to fully explore the whole boundary of the confidence region of $\widehat{\boldsymbol \beta}$, as well as an accurate estimate of the asymptotic distribution of $\widehat{\boldsymbol \beta}$. In our fully synthetic simulation, our hypothesis is that the over-coverage of the bootstrap CI is mainly due to the over-estimation of the variance for $\widehat{\boldsymbol \beta}$.

\begin{table}[!ht]
	\centering\small
	\begin{tabular}{c c c c c c c c}
		\toprule
		         & \multicolumn{1}{c}{$\widehat{\boldsymbol \beta}$} & \multicolumn{4}{c}{$\widehat\REV$}                                            \\
		\cmidrule(lr){2-2} \cmidrule(lr){3-6}
		$\alpha$ & coverage                            & CI width                           & CI width (b) & coverage & coverage (b) & \\
		\midrule
		100/1100 & 0.993                               & 0.132                              & 0.043        & 1.0      & 1.0            \\
		200/1200 & 0.994                               & 0.141                              & 0.059        & 1.0      & 1.0            \\
		300/1300 & 0.980                               & 0.107                              & 0.059        & 1.0      & 1.0            \\
		400/1400 & 0.983                               & 0.098                              & 0.064        & 1.0      & 1.0            \\
		500/1500 & 0.971                               & 0.108                              & 0.069        & 1.0      & 1.0            \\
		\bottomrule
	\end{tabular}
	\caption{Coverage of $\widehat{\boldsymbol \beta}$ and revenue estimates in fully synthetic experiments. All quantities are averaged over 100 simulations for each $\alpha$. The coverage of $\widehat{\boldsymbol \beta}$ is averaged over all components of $\widehat{\boldsymbol \beta}$. For revenue estimates, the columns with "(b)" represent the quantities from the bootstrap CI, while the columns without "(b)" are for the CI from \cref{eq: revenue_ci}. The CI widths are normalized by the revenue from the limit market $\cM\sa$. $\alpha$ is expressed as the ratio of the number of bad items and the total items.}
	\label{tab:full_synthetic_revenue_coverage}
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{ci_width_vs_n_items_full_synthetic.eps}
	\caption{Revenue confidence intervals as a function of the number of items. The analytic CI comes from \cref{eq: revenue_ci}. The true value is the debiased surrogates for revenue in the limit market with interference $\cM\sa$. }
	\label{fig:sim_convergence}
\end{figure}

\subsection{Semi-synthetic experiments}
We perform semi-synthetic experiments almost in the same way as with fully synthetic ones. The difference is that values are sampled from historical bidding data, making the budget and value distributions heavy-tailed. This matches real-world applications better, instead of the uniform distributions of the fully synthetic experiments. More specifically, we first sample a certain number of auctions. For each auction, we sample a given number of advertisers with their per-impression bids. Advertisers that are sampled across different auctions are treated as the same buyers and their budgets are determined by aggregating their values over auctions up to a scalar to calibrated
to get the percentage of budget-constrained buyers equal to what was observed in the real-world auction market, along the same lines as the experiments of \citet{conitzer2022multiplicative}.

We observe similar results in terms of biases as in the fully synthetic experiments. The biases of the debiased surrogates are smaller than those from the limit market with interference $\cM\sa$, with similar bias-$\alpha$ curves as shown in \cref{fig:sim_bias}. Coverage estimates for $\widehat{\boldsymbol \beta}$ and $\widehat\REV$ are shown in \cref{tab:semi_synthetic_revenue_coverage}. The CI from \cref{eq: revenue_ci} is still very conservative as expected, achieving 100\% coverage for all $\alpha$. However, unlike the fully synthetic experiment, the coverage for $\widehat{\boldsymbol \beta}$ is slightly smaller than the nominal level, as well as the coverage of the bootstrap CI of revenue. The under-coverage for $\widehat{\boldsymbol \beta}$ is mainly driven by the under-estimation of the variance of $\widehat{\boldsymbol \beta}$, while the under-coverage of the bootstrap CI for revenue can also be partially attributed to the higher dimensionality (with 40 buyers), making the bootstrap resampling harder to explore the whole space. Although the proposed variance estimator has good asymptotic properties, the results from both the fully and semi- synthetic experiments suggest that it can perform badly, in either direction, for finite markets. Constructing more accurate variance estimators for our debiased estimator in finite settings would certainly mitigate the over- or under-coverage issues that we observe here and deserve more future research. One promising alternative is to construct the CI for $\widehat{\boldsymbol \beta}$ and $\widehat\REV$ by directly bootstrapping the observed value matrix, though this might work best in a setting where the limit market has independent valuations across buyers.

\begin{table}[!ht]
	\centering\small
	\begin{tabular}{c c c c c c c}
		\toprule
		           & \multicolumn{1}{c}{$\widehat{\boldsymbol \beta}$} & \multicolumn{4}{c}{$\widehat\REV$}                                            \\
		\cmidrule(lr){2-2} \cmidrule(lr){3-6}
		$\alpha$   & coverage                            & CI width                           & CI width (b) & coverage & coverage (b) & \\
		\midrule
		1000/11000 & 0.877                               & 0.244                              & 0.044        & 1.0      & 0.95           \\
		2000/12000 & 0.849                               & 0.225                              & 0.043        & 1.0      & 0.87           \\
		3000/13000 & 0.852                               & 0.210                              & 0.041        & 1.0      & 0.81           \\
		4000/14000 & 0.828                               & 0.200                              & 0.040        & 1.0      & 0.90           \\
		5000/15000 & 0.826                               & 0.191                              & 0.039        & 1.0      & 0.90           \\
		\bottomrule
	\end{tabular}
	\caption{Coverage of $\widehat{\boldsymbol \beta}$ and revenue estimates in the semi-synthetic experiments. All quantities are averaged over 100 simulations for each $\alpha$ (the ratio of the number of bad items and the total items). The coverage of $\widehat{\boldsymbol \beta}$ is averaged over all components of $\widehat{\boldsymbol \beta}$. For revenue estimates, the columns with "(b)" represent the quantities from the bootstrap CI, while the columns without "(b)" are for the CI from \cref{eq: revenue_ci}. The CI widths are normalized by the revenue from the limit market $\cM\sa$.}
	\label{tab:semi_synthetic_revenue_coverage}
\end{table}

==> old_intro.tex <==
\section{Introduction}\label{sec:intro}

Online A/B testing, or \emph{experimentation}, is widely used in the internet industry. Major tech companies conduct a large number of A/B tests annually to inform decisions related to ads delivery, online auction mechanisms, user interface components, new feature rollouts, infrastructure improvements, and many other aspects of their products and services.
In the context of online auctions in marketplaces, where buyers bid for sellers' items or advertisers bid for users' impressions, \textit{budget-controlled A/B testing} is a popular tool used e.g. at LinkedIn, Google, and Meta \citep{Basse2016,Liu2021}. The primary advantage of budget control in A/B testing is that it eliminates interference between the A and B groups that could otherwise bias the results: In a traditional A/B test, the budget of a buyer is distributed across all auctions, involving users from both A and B groups. This couples the behavior of the buyer across the groups; for example, increased expenditure under B might decrease expenditure in A, causing interference. However, in a budget-controlled A/B test, each buyer spends half of their budget on users from the A group and the other half on users from the B group, creating two separate but mirrored markets, thus removing the interference caused by a shared budget constraint. % This experiment type, therefore, is commonly used to test various ads delivery changes, such as pacing algorithms (see Section~\ref{ssec:relatedwork}).

Despite clear advantages of budget-controlled A/B testing, they are highly constrained on throughput: only one A/B test can be performed at a time with a single pair of mirrored markets.
% companies are extremely constrained by the number of such experiments they can run; in principle only one experiment can be run at a time if we : buyers (advertisers) can only be charged once for the same item (impression), it is thus not feasible to create additional experimentation throughput by reshuffling users between the A and B groups. An alternative idea is to 
To address this, companies can create more budget splits so more treatments can be tested at the same time. However, this lowers the per-group budget substantially, which could lead to equilibrium distortions and may disproportionately affect smaller buyers. In addition, it poses challenges with respect to statistical power, in view of the fact that tech companies primarily focus on down-funnel conversion events which are difficult to measure effects on to begin with. % In fact, the lack of bandwidth for budget-controlled A/B tests has become one of the major bottlenecks in experimentation for the internet industry.

An alternative approach to increase throughput is market segmentation, which is the focus of this paper. If the overall market can be divided into several relatively isolated submarkets, budget-controlled A/B tests can be conducted in parallel within these submarkets. However, this method also presents some challenges. First, submarkets are rarely completely isolated; certain items may attract buyers from multiple submarkets, resulting in interference across
submarkets when conducting tests in parallel. Second, submarkets differ in terms of buyer (and user) compositions, which might cause the local treatment effect estimates being not representative of the global treatment effect where all buyers are included in the market. The second challenge is relatively easy to address in practice by imposing balancing constraints in the clustering algorithm used to define submarkets, while the first challenge is more fundamentally important and requires deeper theoretical understanding.


As a motivating example, \cref{figmotivation} shows sign consistency betweeen the results of parallel budget-controlled A/B tests (vertical axis) and those obtained from running traditional budget-controlled A/B tests on the entire market (horizontal axis). The figure reports a normalized version of one of the real experiment metrics at Meta, with each submarket covering approximately 6-8\% of advertisers and each experiment condition covering 30\% of users. All submarkets are carefully created with limited imbalances in advertiser composition. We consider 16 different \todo{lf: why are there more than 16 dots in the plot below }treatments, most of which are related to the pacing algorithm, each run for about 6 days, resulting in a total of 99 daily comparisons as presented in \cref{figmotivation}. The benchmark for sign-consistency at a 90\% significance level (for neutral true effects) is 81.5\%. The observed sign consistency rate between the parallel and the traditional budget-controlled experiments is only slightly lower, at around 75\%. Our focus on sign consistency in this context is intentional because it directly relates to the frequency of production decision reversals, which we aim to minimize as much as possible.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=.4]{exp_all_daily.png}
%     \caption{Submarket vs.\ standard budget-controlled A/B test, daily treatment effect. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.
%     }
%     \label{figmotivation}
% \end{figure}
\begin{figure}[ht]
	\centering
	\subfigure[All datapoints.\label{figmotivation}]{\includegraphics[width=0.34\linewidth]{figs/metric2_before_guardrail.png}}\qquad\qquad
	\subfigure[After guardrail metric thresholding. Note the different axis scale.\label{fig:figgood}]{\includegraphics[width=0.34\linewidth]{figs/metric2_after_guardrail.png}}
	\label{noteneeded}
	\caption{Parallel vs.\ standard budget-controlled A/B test, daily treatment effect. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.}
\end{figure}

% As discussed in Section~\ref{sec:intro}, we analyze 16 real treatments at Meta. For each treatment, we set up two experiments: one is a parallel budget-controlled A/B test ($\alpha>0$) and the other is the standard budget-controlled A/B test on the entire market ($\alpha=0$). Two experiments, which we call a combo, are run during the same time period. The submarkets are formed using a balanced partitioning algorithm for a bipartite graph that connects advertisers and users' auctions to maximize auction purity, with constraints on a selective set of advertiser features (e.g., country, budget, optimization goals, etc.) so as to evenly distribute advertisers among the resulting submarkets. 

% We stress that all production submarket experiments considered at Meta use naive treatment effect estimator, not the proposed de-biasing procedure due to the theoretical challenges discussed in Section~\ref{ssc:inropractice} when it comes to production environment and a series of infrastructural and scalability limitations. However, the asymptotic theories remain highly valuable, since they provides a formal understanding on the magnitude of interference bias, which allows us to make more informed product decisions under such settings.

\cref{tab:sign_consistency} shows the sign consistency rate of comparisons for daily and 6-day aggregated results, including for a second metric. Since submarkets are not perfectly isolated, we use a guardrail metric to measure the interference between submarkets, and use a threshold on the guardrail metric to improve reliability. As seen in \cref{tab:sign_consistency}, by eliminating experiments where the guardrail metric violates the threshold, we meaningfully improve the consistency rate for both metrics in daily and 6-day results. In practice, approximately 10\% of submarket experiments violate the guardrail threshold. \cref{fig:figgood} demonstrates the treatment effect comparisons for daily results after we remove such data points. The results are generally satisfactory, however the existence of biases is evident even after removing data points that violated the guardrail threshold.
%low-quality estimates (e.g., those that deviate further from the 45-degree line).
Evidently, quantitatively understanding the interference bias to improve the accuracy of the estimates is conducive to better decisions, and that is what we set to do in this work.

\begin{table}[ht]
	\centering\small
	\caption{Sign consistency between submarket and standard budget-controlled A/B test}
	\begin{tabular}{ccccc}
		\hline
		\multirow{2}{*}{Duration} & \multirow{2}{*}{Data} & \multirow{2}{*}{Num} & \multicolumn{2}{c}{Sign consistency (\%)}            \\
		                          &                       &                      & Metric 1                                  & Metric 2 \\
		\hline
		6 days                    & All combos            & 16                   & 87.5                                      & 68.8     \\

		6 days                    & within guardrail      & 14                   & 100                                       & 78.6     \\

		1 day                     & All combos            & 99                   & 75.8                                      & 73.7     \\

		1 day                     & within guardrail      & 84                   & 81.0                                      & 76.2     \\
		\hline
	\end{tabular}
	\label{tab:sign_consistency}
\end{table}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=.4]{exp_no_imp_shift_daily.png}
%     \caption{Submarket vs.\ standard budget-controlled A/B test, daily treatment effect. All data points that violate the guardrail threshold are removed. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.
%     }
%     \label{fig:figgood}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_all.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_no_imp_shift.png}
%     \end{subfigure}
%     \caption{submarket vs standard budget-controlled A/B test, 6-day treatment effect. The neutral treatment effect is represented by a value of 1.0. For example, 1.01 can be interpreted as 1\% treatment effect. Red crosses indicate instances of sign inconsistencies. The upper two figures present all combos while the lower two only present combos without significant impression shift.}
%     \label{fig:6daycompare}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_all_daily.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_no_imp_shift_daily.png}
%     \end{subfigure}
%     \caption{submarket vs standard budget-controlled A/B test, daily treatment effect. The neutral treatment effect is represented by a value of 1.0. For example, 1.01 can be interpreted as 1\% treatment effect. Red crosses indicate instances of sign inconsistencies. The upper two figures present all combos while the lower two only present combos without significant impression shift.}
%     \label{fig:1daycompare}
% \end{figure}


The contributions of this paper are as follows. First, we introduce and demonstrate the effectiveness of the parallel budget-controlled A/B test design with submarkets in Meta's production environment, which, to our best knowledge, is a novel approach. Second, we formally define market interference in first-price auction markets using the First Price Pacing Equilibrium (FPPE) framework \citep{conitzer2022pacing}. Third, we propose a debiased surrogate that eliminates the first-order bias of FPPE, drawing upon the principles of sensitivity analysis in mathematical programs \citep{shapiro2021lectures}. Fourth, we derive a plug-in estimator for the surrogate and establish its asymptotic normality. Fifth, we provide an estimation procedure for submarket parallel budget-controlled A/B tests. Finally, we present numerical examples on semi-synthetic data, confirming that the debiasing technique achieves the desired coverage properties.
%\cref{sec:conclusion} concludes.

% Section~\ref{sec:theoryoverview} introduces the FPPE framework. The formal problem setup is given in Section~\ref{sec:setup}. Asymptotic theories around FPPE are presented in Section~\ref{sec:results}. Section~\ref{sec:ABTest} formalizes the parallel A/B testing problem under interference and provides the estimation procedure. Numerical examples on synthetic and semi-synthetic data are presented in Section~\ref{sec:exp}. We conclude in Section~\ref{sec:conclusion}.

\subsection{Parallel A/B Testing in Practice}\label{ssc:inropractice}
In this section we describe the real-world problem of A/B testing that we wish to model, and our proposed solution of parallel A/B tests in carefully balanced submarkets; the formal model appears in \Cref{sec:theoryoverview} and \Cref{sec:setup}. Along with the description of the real-world problem, we will also discuss which aspects of it will be or will not be captured by our theoretical model.

We start by describing the market environment. Assume that there is a set of $n$ advertisers, and each advertiser $i$ has a budget $b_i$. Whenever a user shows up on the platform an \emph{impression opportunity} occurs, and an auction is conducted in order to determine which subset of ads will be shown to the user. Each advertiser $i$ has some stated value $v_{i}(\t)$ of being shown to a particular impression opportunity $\t$. This may not be their true valuation; in practice it may be their stated willingness to pay for a click, multiplied by an estimated click-through-rate for the pair ($i$,$\t$). The advertiser submits a bid which is determined based on $v_{i}(\t)$, as well as the expenditure of the advertiser so far. For example, in \emph{multiplicative pacing}~\citep{balseiro2017budget,conitzer2022multiplicative,conitzer2022pacing}, the platform adaptively learns a \emph{pacing multiplier} $\beta_i\in [0,1]$ such that the bid is formed as $ \beta_i v_{i}(\t)$. The budget-management system then adaptively controls $\beta_i$ over time, in order to ensure the correct rate of budget expenditure on behalf of the advertiser.
\textcolor{red}{[Delete the following? This is explained again below.] The auction format for an impression opportunity is typically some generalization of the first or second-price auction, though the real-world auctions are not fully captured by any simple-to-describe auction model from the literature. For example, in the setting of inserting ads into a news feed, multiple ads may be allowed to be shown, but the exact number may depend on the size of each ad, the size of other content in the feed, and so forth. }

\textcolor{red}{[Can we drastically reduce this paragraph by simply listing the 3 working assumptions and putting all references and explanations to appendix? The information provided here doesn't seem to be a must to define our problem. If we really want readers to understand the rationale behind them, we can point them to the appendix to understand the reasoning for these assumptions?]}In our theoretical model, we will simplify the auction format in three respects:
first, we will assume that each impression opportunity allows exactly one ad to be shown. This is a common assumption in the literature studying both online learning for budget management~\citep{borgs2007dynamics,balseiro2019learning} as well as in the literature on equilibrium outcomes under budget management~\citep{balseiro2017budget,conitzer2022multiplicative,conitzer2022pacing,aggarwal2019autobidding,balseiro2023contextual}.
Thirdly \textcolor{red}{(Second?)}, we assume that each individual auction is a \emph{first-price auction}, meaning that the highest bidder wins, and pays their bid. Internet advertising uses both first and second-price auctions, depending on the particular context~\citep{balseiro2023contextual,goke2021bidders}, though generalizations of the second-price auction are arguably still more common, in particular for sponsored search and feed auctions. We focus on first-price auctions because the equilibrium outcomes under budget management satisfy two crucial properties from the perspective of statistical inference: they are unique, and the equilibrium is captured by a convex program~\citep{conitzer2022pacing}.
In contrast, equilibria under budget management in second-price auctions may not be unique~\citep{conitzer2022multiplicative}, and they are PPAD-hard to compute~\citep{chen2021complexity}. It is an interesting future research direction to figure out how to develop results for the second-price setting, though we expect it to be much harder.
We will also abstract away the dynamic temporal aspects of budget management: instead of the pacing multipliers being learned over time, we will assume that what we observe is the set of pacing multipliers in equilibrium. Secondly \textcolor{red}{(Third)}, in the real world, advertisers may use a variety of budget management algorithms beyond multiplicative pacing. For example, Google also offers \emph{probabilistic throttling}, where bids are not modified, and instead the expenditure is managed by independently flipping a coin for each auction, in order to determine whether to bid at all~\citep{balseiro2017budget,chen2021throttling,karande2013optimizing}.
We assume that every advertiser uses multiplicative pacing in order to manage budgets.
Budget-management equilibria in first-price auctions with probabilistic throttling are known to also be unique and computable~\citep{chen2021throttling}, so it is possible that similar results could be obtained for that setting, though it is not known whether those equilibria are captured by a convex mathematical program, which is a crucial fact for our technical approach.

Now that we have discussed budget management, we describe the A/B testing problem. Suppose that a platform wants to run $K$ A/B tests, which may affect, e.g., the valuations that advertisers have for impression slots, revenue, etc.
Naively performing the A/B test on a per-impression or per-user basis and then simply running the market as usual will not work, because the budget management system means that the A and B users will be affected by each other through the budget coupling.
As mentioned in the introduction, a possible option is to perform budget splitting: create $K+1$ copies of each advertiser (corresponding to each test, as well as a holdout ``A'' control copy), randomize users into one of the $K+1$ markets, and run separate budget management for each copy of the $K+1$ advertisers. As mentioned earlier, this approach runs into problems because small advertisers end up with prohibitively-small budgets, and there is a large negative impact on statistical power because some of the events measured by the A/B tests might be far downstream of an impression. \textcolor{red}{[To reduce duplicate content and make the paragraph shorter, consider the following] Having discussed budget management, we now describe the A/B testing problem. Suppose a platform wants to run $K$ A/B tests that may impact advertiser valuations for impression slots. Simply performing A/B tests on a per-impression or per-user basis as usual won't work due to the budget management system causing A and B groups to affect each other via budget coupling. As discussed in \cref{sec:intro}, the possible solution of budget splitting -- create $K+1$ equal copies of each advertiser (including a control copy), split budget equally across copies, randomize users into the $K+1$ markets, and manage budgets independently in each market -- runs into problems.}

Instead, our paper considers the following parallel A/B test paradigm based on market segmentation.
We first define a bipartite graph between advertisers and users based on targeting criteria. Subsequently, we cluster the advertisers into $K$ clusters, where the objective is to minimize the sum of weighted edges between clusters subject to traffic balancing constraints to make the resulting clusters as similar to the whole market as possible. The edge weight between a pair of advertisers is the number of impressions (or users) where they are both within the top-$k$ bids. The choice of $k$ is a parameter that must be chosen based on experience with the specific application setting.
If the clustering achieves a small objective function value, then each cluster is a mostly isolated submarket, in the sense that each user will mostly receive bids from advertisers in a single cluster.
Then, we run an A/B test within each of the $K$ submarkets.
Every user is randomly assigned to either ``A'' or ``B'' in each submarket.
Note that the same user can be in ``A'' in submarket 1 and ``B'' in submarket 2. This means that all the A/B tests must be mutually compatible; in practice this means that our approach is best suited for A/B tests that apply to advertisers, as opposed to, e.g., user-side user interface changes.
If the interaction between different submarkets is not too strong, then we expect that hypothesis testing in a submarket is indicative of the true treatment effect within that submarket.
Additionally, if each submarket is representative of the overall market, then such a hypothesis test is also indicative of the true treatment effect across the whole market.

In our theoretical model we use a coarser notion of contamination between a pair of submarkets than the top-$k$ measure that  we use in practice, and we measure the number of items with \emph{any} bids from buyers from separate submarkets.
In practice, this measure is too coarse (and often very large). It is an interesting follow-up question to come up with stronger theoretical results that allow for finer-grained measures of contamination.
Secondly, our theoretical model will assume that what we are interested in is the treatment effect within a submarket. This implicitly assumes that each submarket is representative of the overall market.

We survey related works in \cref{ssec:relatedwork}.
\section{Review of FPPE Theory}\label{sec:theoryoverview}


==> simulations_draft.tex <==
% To check if the proposed estimator for $\beta$ (a vector) has less bias than the baseline, we use the root mean square error (RMSE) as the distance metric from the estimates to the true value from limit FPPE. For the coverage of $\beta$, we check if each dimension of $\Tilde\beta^*$ is covered by the confidence interval of $\widehat\beta$ in that dimension, and consider that $\Tilde\beta^*$ is covered when each dimension of $\Tilde\beta^*$ is within its marginal confidence interval of $\widehat\beta$. For revenue (a scalar), we apply the typical absolute error as the distance metric to the true value and check the coverage accordingly. 

% The results are shown in Table~\ref{tab:full_synthetic_beta} for $\beta$ and in Table~\ref{tab:full_synthetic_revenue_bias} and~\ref{tab:full_synthetic_revenue_coverage} for revenue. First of all, for both $\beta$ and revenue, the bias of the debiased estimator is indeed slightly smaller than the baseline estimator. For revenue estimates, we also compare the bootstrap CI and the analytical CI based on $\beta$ marginals. As expected, bootstrap CI has much smaller width but can possibly under cover when the bootstrap samples do not have a good coverage of the whole space. 
% \begin{table} 
%     \centering
%     \begin{tabular}{c c c c c}
%         \toprule
%          $\alpha$ & baseline rmse & debiased rmse & frac less biased & coverage \\
%          \midrule
%          2/202 & 0.315 & 0.304 & 0.98 & 1.0 \\
%          4/204 & 0.122 & 0.120 & 0.73 & 1.0 \\
%          6/206 & 0.159 & 0.151 & 0.90 & 1.0 \\
%          8/208 & 0.130 & 0.127 & 0.81 & 1.0 \\
%          10/210 & 0.112 & 0.106 & 0.95 & 1.0 \\
%          \bottomrule
%     \end{tabular}
%     \caption{Bias and coverage results for $\widehat\beta$. All quantities are averaged over 100 simulations for each $\alpha$. The RMSEs are normalized by the $l2$-norm of the true $\beta$ from the limit FPPE. The 'frac less biased' column shows the fraction of 100 simulations where the debiased estimator has a smaller RMSE than the baseline.}
%     \label{tab:full_synthetic_beta}
% \end{table}

% \begin{table}[!ht] 
%     \centering
%     \begin{tabular}{c c c c c}
%         \toprule
%          $\alpha$ & baseline bias & debiased bias & frac less biased  \\
%          \midrule
%          2/202 & 0.002 & -0.001 & 0.45  \\
%          4/204 & 0.008 & 0.006 & 0.63  \\
%          6/206 & 0.005 & 0.001 & 0.47  \\
%          8/208 & 0.004 & -0.001 & 0.40  \\
%          10/210 & 0.003 & -0.001 & 0.46  \\
%          \bottomrule
%     \end{tabular}
%     \caption{Bias of revenue estimates. All quantities are averaged over 100 simulations for each $\alpha$. The biases are relative to the true revenue from the limit FPPE. The 'frac less biased' column shows the fraction of 100 simulations where the debiased estimator has a smaller bias than the baseline.}
%     \label{tab:full_synthetic_revenue_bias}
% \end{table}

% \begin{table}[!ht] 
%     \centering
%     \begin{tabular}{c c c c c c c}
%         \toprule
%          $\alpha$ & CI width & CI width (b) & coverage & coverage (b) &  \\
%          \midrule
%          2/202 & 0.334 & 0.097 & 1.0 & 0.99 \\
%          4/204 & 0.327 & 0.074 & 1.0 & 0.98 \\
%          6/206 & 0.319 & 0.079 & 1.0 & 0.96 \\
%          8/208 & 0.320 & 0.084 & 1.0 & 0.99 \\
%          10/210 & 0.277 & 0.081 & 1.0 & 0.98 \\
%          \bottomrule
%     \end{tabular}
%     \caption{Coverage of revenue estimates. All quantities are averaged over 100 simulations for each $\alpha$. The columns with "(b)" represents the quantities from the bootstrap CI. The CI widths are relative to the true revenue from the limit FPPE.}
%     \label{tab:full_synthetic_revenue_coverage}
% \end{table}

==> text/intro_long.tex <==

Online A/B testing, or \emph{experimentation}, is widely used in the internet industry. Major tech companies conduct a large number of A/B tests annually to inform decisions related to ads delivery, online auction mechanisms, user interface components, new feature rollouts, infrastructure improvements, and many other aspects of their products and services.
In the context of online auctions in marketplaces, where buyers bid for sellers' items or advertisers bid for users' impressions, \textit{budget-controlled A/B testing} is a popular tool used e.g. at LinkedIn, Google, and Meta \citep{Basse2016,Liu2021}. The primary advantage of budget control in A/B testing is that it eliminates interference between the A and B groups that could otherwise bias the results: In a traditional A/B test, the budget of a buyer is distributed across all auctions, involving users from both A and B groups. This couples the behavior of the buyer across the groups; for example, increased expenditure under B might decrease expenditure in A, causing interference. However, in a budget-controlled A/B test, each buyer spends half of their budget on users from the A group and the other half on users from the B group, creating two separate but mirrored markets, thus removing the interference caused by a shared budget constraint. % This experiment type, therefore, is commonly used to test various ads delivery changes, such as pacing algorithms (see Section~\ref{ssec:relatedwork}).

Despite clear advantages of budget-controlled A/B testing, they are highly constrained on throughput: only one A/B test can be performed at a time with a single pair of mirrored markets.
% companies are extremely constrained by the number of such experiments they can run; in principle only one experiment can be run at a time if we : buyers (advertisers) can only be charged once for the same item (impression), it is thus not feasible to create additional experimentation throughput by reshuffling users between the A and B groups. An alternative idea is to 
To address this, companies can create more budget splits so more treatments can be tested at the same time. However, this lowers the per-group budget substantially, which could lead to equilibrium distortions and may disproportionately affect smaller buyers. In addition, it poses challenges with respect to statistical power, in view of the fact that tech companies primarily focus on down-funnel conversion events which are difficult to measure effects on to begin with. % In fact, the lack of bandwidth for budget-controlled A/B tests has become one of the major bottlenecks in experimentation for the internet industry.

An alternative approach to increase throughput is market segmentation, which is the focus of this paper. If the overall market can be divided into several relatively isolated submarkets, budget-controlled A/B tests can be conducted in parallel within these submarkets. However, this method also presents some challenges. First, submarkets are rarely completely isolated; certain items may attract buyers from multiple submarkets, resulting in interference across
submarkets when conducting tests in parallel. Second, submarkets differ in terms of buyer (and user) compositions, which might cause the local treatment effect estimates being not representative of the global treatment effect where all buyers are included in the market. The second challenge is relatively easy to address in practice by imposing balancing constraints in the clustering algorithm used to define submarkets, while the first challenge is more fundamentally important and requires deeper theoretical understanding.


As a motivating example, \cref{figmotivation} shows sign consistency betweeen the results of parallel budget-controlled A/B tests (vertical axis) and those obtained from running traditional budget-controlled A/B tests on the entire market (horizontal axis). The figure reports a normalized version of one of the real experiment metrics at Meta, with each submarket covering approximately 6-8\% of advertisers and each experiment condition covering 30\% of users. All submarkets are carefully created with limited imbalances in advertiser composition. We consider 16 different \todo{lf: why are there more than 16 dots in the plot below }treatments, most of which are related to the pacing algorithm, each run for about 6 days, resulting in a total of 99 daily comparisons. The benchmark for sign-consistency at a 90\% significance level (for neutral true effects) is 81.5\%. The observed sign consistency rate between the parallel and the traditional budget-controlled experiments is only slightly lower, at around 75\%. Our focus on sign consistency in this context is intentional because it directly relates to the frequency of production decision reversals, which we aim to minimize as much as possible.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=.4]{exp_all_daily.png}
%     \caption{Submarket vs.\ standard budget-controlled A/B test, daily treatment effect. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.
%     }
%     \label{figmotivation}
% \end{figure}
\begin{figure}[ht]
	\centering
	\subfigure[All datapoints.\label{figmotivation}]{\includegraphics[width=0.34\linewidth]{figs/metric2_before_guardrail.png}}\qquad\qquad
	\subfigure[After guardrail metric thresholding. Note the different axis scale.\label{fig:figgood}]{\includegraphics[width=0.34\linewidth]{figs/metric2_after_guardrail.png}}
	\label{noteneeded}
	\caption{Parallel vs.\ standard budget-controlled A/B test, daily treatment effect. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.}
\end{figure}

% As discussed in Section~\ref{sec:intro}, we analyze 16 real treatments at Meta. For each treatment, we set up two experiments: one is a parallel budget-controlled A/B test ($\alpha>0$) and the other is the standard budget-controlled A/B test on the entire market ($\alpha=0$). Two experiments, which we call a combo, are run during the same time period. The submarkets are formed using a balanced partitioning algorithm for a bipartite graph that connects advertisers and users' auctions to maximize auction purity, with constraints on a selective set of advertiser features (e.g., country, budget, optimization goals, etc.) so as to evenly distribute advertisers among the resulting submarkets. 

% We stress that all production submarket experiments considered at Meta use naive treatment effect estimator, not the proposed de-biasing procedure due to the theoretical challenges discussed in Section~\ref{ssc:inropractice} when it comes to production environment and a series of infrastructural and scalability limitations. However, the asymptotic theories remain highly valuable, since they provides a formal understanding on the magnitude of interference bias, which allows us to make more informed product decisions under such settings.

\cref{tab:sign_consistency} shows the sign consistency rate of comparisons for daily and 6-day aggregated results, including for a second metric. Since submarkets are not perfectly isolated, we use a guardrail metric to measure the interference between submarkets, and use a threshold on the guardrail metric to improve reliability. As seen in \cref{tab:sign_consistency}, by eliminating experiments where the guardrail metric violates the threshold, we meaningfully improve the consistency rate for both metrics in daily and 6-day results. In practice, approximately 10\% of submarket experiments violate the guardrail threshold. \cref{fig:figgood} demonstrates the treatment effect comparisons for daily results after we remove such data points. The results are generally satisfactory, however the existence of biases is evident even after removing data points that violated the guardrail threshold.
%low-quality estimates (e.g., those that deviate further from the 45-degree line).
Evidently, quantitatively understanding the interference bias to improve the accuracy of the estimates is conducive to better decisions, and that is what we set to do in this work.

\begin{table}[ht]
	\centering\small
	\caption{Sign consistency between submarket and standard budget-controlled A/B test}
	\begin{tabular}{ccccc}
		\hline
		\multirow{2}{*}{Duration} & \multirow{2}{*}{Data} & \multirow{2}{*}{Num} & \multicolumn{2}{c}{Sign consistency (\%)}            \\
		                          &                       &                      & Metric 1                                  & Metric 2 \\
		\hline
		6 days                    & All combos            & 16                   & 87.5                                      & 68.8     \\

		6 days                    & within guardrail      & 14                   & 100                                       & 78.6     \\

		1 day                     & All combos            & 99                   & 75.8                                      & 73.7     \\

		1 day                     & within guardrail      & 84                   & 81.0                                      & 76.2     \\
		\hline
	\end{tabular}
	\label{tab:sign_consistency}
\end{table}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=.4]{exp_no_imp_shift_daily.png}
%     \caption{Submarket vs.\ standard budget-controlled A/B test, daily treatment effect. All data points that violate the guardrail threshold are removed. We denote neutral treatment effects with a value of $1.0$. For example, $1.01$ can be interpreted as $1\%$ treatment effect. Red crosses indicate instances of sign inconsistencies.
%     }
%     \label{fig:figgood}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_all.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_no_imp_shift.png}
%     \end{subfigure}
%     \caption{submarket vs standard budget-controlled A/B test, 6-day treatment effect. The neutral treatment effect is represented by a value of 1.0. For example, 1.01 can be interpreted as 1\% treatment effect. Red crosses indicate instances of sign inconsistencies. The upper two figures present all combos while the lower two only present combos without significant impression shift.}
%     \label{fig:6daycompare}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_all_daily.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=.4]{exp_no_imp_shift_daily.png}
%     \end{subfigure}
%     \caption{submarket vs standard budget-controlled A/B test, daily treatment effect. The neutral treatment effect is represented by a value of 1.0. For example, 1.01 can be interpreted as 1\% treatment effect. Red crosses indicate instances of sign inconsistencies. The upper two figures present all combos while the lower two only present combos without significant impression shift.}
%     \label{fig:1daycompare}
% \end{figure}


The contributions of this paper are as follows. First, we introduce and demonstrate the effectiveness of the parallel budget-controlled A/B test design with submarkets in Meta's production environment, which, to our best knowledge, is a novel approach. Second, we formally define market interference in first-price auction markets using the First Price Pacing Equilibrium (FPPE) framework \citep{conitzer2022pacing}. Third, we propose a debiased surrogate that eliminates the first-order bias of FPPE, drawing upon the principles of sensitivity analysis in mathematical programs \citep{shapiro2021lectures}. Fourth, we derive a plug-in estimator for the surrogate and establish its asymptotic normality. Fifth, we provide an estimation procedure for submarket parallel budget-controlled A/B tests. Finally, we present numerical examples on semi-synthetic data, confirming that the debiasing technique achieves the desired coverage properties.
%\cref{sec:conclusion} concludes.

% Section~\ref{sec:theoryoverview} introduces the FPPE framework. The formal problem setup is given in Section~\ref{sec:setup}. Asymptotic theories around FPPE are presented in Section~\ref{sec:results}. Section~\ref{sec:ABTest} formalizes the parallel A/B testing problem under interference and provides the estimation procedure. Numerical examples on synthetic and semi-synthetic data are presented in Section~\ref{sec:exp}. We conclude in Section~\ref{sec:conclusion}.

\subsection{Parallel A/B Testing in Practice}\label{ssc:inropractice}
In this section we describe the real-world problem of A/B testing that we wish to model, and our proposed solution of parallel A/B tests in carefully balanced submarkets; the formal model appears in \Cref{sec:theoryoverview} and \Cref{sec:setup}. Along with the description of the real-world problem, we will also discuss which aspects of it will be or will not be captured by our theoretical model.

We start by describing the market environment. Assume that there is a set of $n$ advertisers, and each advertiser $i$ has a budget $b_i$. Whenever a user shows up on the platform an \emph{impression opportunity} occurs, and an auction is conducted in order to determine which subset of ads will be shown to the user. Each advertiser $i$ has some stated value $v_{i}(\t)$ of being shown to a particular impression opportunity $\t$. This may not be their true valuation; in practice it may be their stated willingness to pay for a click, multiplied by an estimated click-through-rate for the pair ($i$,$\t$). The advertiser submits a bid which is determined based on $v_{i}(\t)$, as well as the expenditure of the advertiser so far. For example, in \emph{multiplicative pacing}~\citep{balseiro2017budget,conitzer2022multiplicative,conitzer2022pacing}, the platform adaptively learns a \emph{pacing multiplier} $\beta_i\in [0,1]$ such that the bid is formed as $ \beta_i v_{i}(\t)$. The budget-management system then adaptively controls $\beta_i$ over time, in order to ensure the correct rate of budget expenditure on behalf of the advertiser.
The auction format for an impression opportunity is typically some generalization of the first or second-price auction, though the real-world auctions are not fully captured by any simple-to-describe auction model from the literature. For example, in the setting of inserting ads into a news feed, multiple ads may be allowed to be shown, but the exact number may depend on the size of each ad, the size of other content in the feed, and so forth.

In our theoretical model, we will simplify the auction format in three respects:
first, we will assume that each impression opportunity allows exactly one ad to be shown. This is a common assumption in the literature studying both online learning for budget management~\citep{borgs2007dynamics,balseiro2019learning} as well as in the literature on equilibrium outcomes under budget management~\citep{balseiro2017budget,conitzer2022multiplicative,conitzer2022pacing,aggarwal2019autobidding,balseiro2023contextual}.
Thirdly, we assume that each individual auction is a \emph{first-price auction}, meaning that the highest bidder wins, and pays their bid. Internet advertising uses both first and second-price auctions, depending on the particular context~\citep{balseiro2023contextual,goke2021bidders}, though generalizations of the second-price auction are arguably still more common, in particular for sponsored search and feed auctions. We focus on first-price auctions because the equilibrium outcomes under budget management satisfy two crucial properties from the perspective of statistical inference: they are unique, and the equilibrium is captured by a convex program~\citep{conitzer2022pacing}.
In contrast, equilibria under budget management in second-price auctions may not be unique~\citep{conitzer2022multiplicative}, and they are PPAD-hard to compute~\citep{chen2021complexity}. It is an interesting future research direction to figure out how to develop results for the second-price setting, though we expect it to be much harder.
We will also abstract away the dynamic temporal aspects of budget management: instead of the pacing multipliers being learned over time, we will assume that what we observe is the set of pacing multipliers in equilibrium. Secondly, in the real world, advertisers may use a variety of budget management algorithms beyond multiplicative pacing. For example, Google also offers \emph{probabilistic throttling}, where bids are not modified, and instead the expenditure is managed by independently flipping a coin for each auction, in order to determine whether to bid at all~\citep{balseiro2017budget,chen2021throttling,karande2013optimizing}.
We assume that every advertiser uses multiplicative pacing in order to manage budgets.
Budget-management equilibria in first-price auctions with probabilistic throttling are known to also be unique and computable~\citep{chen2021throttling}, so it is possible that similar results could be obtained for that setting, though it is not known whether those equilibria are captured by a convex mathematical program, which is a crucial fact for our technical approach.

Now that we have discussed budget management, we describe the A/B testing problem. Suppose that a platform wants to run $K$ A/B tests, which may affect, e.g., the valuations that advertisers have for impression slots, revenue, etc.
Naively performing the A/B test on a per-impression or per-user basis and then simply running the market as usual will not work, because the budget management system means that the A and B users will be affected by each other through the budget coupling.
As mentioned in the introduction, a possible option is to perform budget splitting: create $K+1$ copies of each advertiser (corresponding to each test, as well as a holdout ``A'' control copy), randomize users into one of the $K+1$ markets, and run separate budget management for each copy of the $K+1$ advertisers. As mentioned earlier, this approach runs into problems because small advertisers end up with prohibitively-small budgets, and there is a large negative impact on statistical power because some of the events measured by the A/B tests might be far downstream of an impression.

Instead, our paper considers the following parallel A/B test paradigm based on market segmentation.
We first define a bipartite graph between advertisers and users based on targeting criteria. Subsequently, we cluster the advertisers into $K$ clusters, where the objective is to minimize the sum of weighted edges between clusters subject to traffic balancing constraints to make the resulting clusters as similar to the whole market as possible. The edge weight between a pair of advertisers is the number of impressions (or users) where they are both within the top-$k$ bids. The choice of $k$ is a parameter that must be chosen based on experience with the specific application setting.
If the clustering achieves a small objective function value, then each cluster is a mostly isolated submarket, in the sense that each user will mostly receive bids from advertisers in a single cluster.
Then, we run an A/B test within each of the $K$ submarkets.
Every user is randomly assigned to either ``A'' or ``B'' in each submarket.
Note that the same user can be in ``A'' in submarket 1 and ``B'' in submarket 2. This means that all the A/B tests must be mutually compatible; in practice this means that our approach is best suited for A/B tests that apply to advertisers, as opposed to, e.g., user-side user interface changes.
If the interaction between different submarkets is not too strong, then we expect that hypothesis testing in a submarket is indicative of the true treatment effect within that submarket.
Secondly, if each submarket is representative of the overall market, then such a hypothesis test is also indicative of the true treatment effect across the whole market.

In our theoretical model we use a coarser notion of contamination between a pair of submarkets than the top-$k$ measure that  we use in practice. In our theoretical model, we measure the number of items with \emph{any} bids from buyers from separate submarkets.
In practice, this measure is too coarse (and often very large). It is an interesting follow-up question to come up with stronger theoretical results that allow for finer-grained measures of contamination.
Secondly, our theoretical model will assume that what we are interested in is the treatment effect within a submarket. This implicitly assumes that each submarket is representative of the overall market.

We survey related works in \cref{ssec:relatedwork}.
\section{Review of FPPE Theory}\label{sec:theoryoverview}

